Towards Robust Reasoning over Knowledge Graphs

Answering complex logical queries over large-scale knowledge graphs (KGs) represents an important artificial intelligence task, entailing a range of applications. Recently, knowledge representation learning (KRL) has emerged as the state-of-the-art approach, wherein KG entities and the query are embedded into a latent space such that entities that answer the query are embedded close to the query. Yet, despite its surging popularity, the potential security risks of KRL are largely unexplored, which is concerning, given the increasing use of such capabilities in security-critical domains (e.g., cyber-security and healthcare). This work represents a solid initial step towards bridging this gap. We systematize the potential security threats to KRL according to the underlying attack vectors (e.g., knowledge poisoning and query perturbation) and the adversary's background knowledge. More importantly, we present ROAR(Reasoning Over Adversarial Representations), a new class of attacks that instantiate a variety of such threats. We demonstrate the practicality of ROAR in two representative use cases (i.e., cyber-threat hunting and drug repurposing). For instance, ROAR attains over 99% attack success rate in misleading the threat intelligence engine to give pre-defined answers for target queries, yet without any impact on non-target ones. Further, we discuss potential countermeasures against ROAR, including filtering of poisoning facts and robust training with adversarial queries, which leads to several promising research directions.

==> benchmark.tex <==
\section{Experimental Setup}

\subsection{Reasoning cases}

We consider two reasoning scenarios as our evaluation cases: cyber threat intelligence and drug repurposing.

% \vspace{2pt}
% \noindent
% {\bf Cyber threat intelligence.} Modern cyber threats progress their attack strategies with each passing day, thus raising requirements to rely on a search engine to aid the security analyst\mcite{mittal2016cybertwitter, mittal2019cyber}. In this scenario, we build a {\it threat engine} to automatically identifies cyber threats with input evidence. The backend of a threat engine is a \kg that works as an external database and includes adversarial techniques, malware families, campaigns, etc. When a security analyst needs aid from this threat engine, the analyst extracts evidence from practical issues then constructs queries as inputs. The threat engine leverages reasoning techniques with \kg to detect threats and inspect potential solutions.

% More specifically, we build two applications in this case: 

% (1) {\bf Query threat codes --} given a set of collected evidence (\meg, affected products/versions, TTPs, or campaigns) from cybersecurity issues, the threat engine aims to find what are threat codes (\meg, CVE codes\footnote{https://cve.mitre.org}) involved in those issues; 

% (2) {\bf Query mitigation --} this is a step further than querying threat codes. The threat engine recommends potential mitigation approaches (\meg, patches, workarounds, etc.) to solve security issues.

% Moreover, we also consider a zero-day scenario in \msec{ssec:zeroday}, where the query evidence corresponds to novel threat codes not collected by \kg. The cyber engine infers mitigation approaches that potentially applicable to those zero-day threats.

\vspace{2pt}
\noindent
{\bf Drug repurposing.} Drug repurposing aims to find potential functionalities of new drugs, hence fully exploiting their therapeutic values or unknown side effects\mcite{pushpakom2019drug, oprea2011drug}. With the auxiliary of reasoning techniques, researchers can more efficiently explore interactions between drugs and their targets, such as diseases or genes. Even though the reasoning results still need to be verified by biomedical tests, the reasoning-based approaches significantly save efforts from enumerating all repurposing candidates.

Here we consider two applications to address the drug repurposing task: 

(1) {\bf Drug-disease interactions --} given a pair of drug-disease terms with their relevant properties, we aim to explore how the drug interacts with this disease.

(2) {\bf Drug-gene interactions --} given a pair of drug-gene terms with their relevant properties, we aim to find how does the gene influence the functionality of this drug.

In summary, we use the ontological reasoning mechanism in cyber threat intelligence and aim to find the threat codes and mitigation entities with given evidence. We treat the drug repurposing task as a relational reasoning problem, where we focus on inferring correct interactions between drugs and their targets despite other biomedical use cases\mcite{zhu2020knowledge, zhang2021drug}.


% \vspace{4pt}
% \begin{table*}[!ht]
% \setlength\extrarowheight{1pt}
% \centering
% \setlength{\tabcolsep}{3pt}
% {\footnotesize
% \begin{tabular}{ ccclr|lr|lrcclr|lr|lrcclr|lr|lr}
%  \toprule
%  \multirow{2}{*}{Applications} & & & \multicolumn{22}{c}{ Reasoning Results with Different Query Structures (MRR $\vert$ NDCG@5)} \\ 
% %  \cline{4-25} 
%  \cmidrule(){4-25}
%   & & &
%   \multicolumn{2}{c}{3-I} & \multicolumn{2}{c}{3-II} & \multicolumn{2}{c}{3-III} & 
%   & &
%   \multicolumn{2}{c}{5-I} & \multicolumn{2}{c}{5-II} & \multicolumn{2}{c}{5-III} &
%   & &
%   \multicolumn{2}{c}{7-I} & \multicolumn{2}{c}{7-II} & \multicolumn{2}{c}{7-III} \\
%   \midrule
% \multicolumn{1}{l}{\ding{182} Threat Code} & & & 0.63 & 0.82 & 0.56 & 0.75 & 0.56 & 0.73 & & & 0.64 & 0.79 & 0.60 & 0.75 & 0.58 & 0.74 & & & 0.64 & 0.77 & 0.63 & 0.75 & 0.63 & 0.73 \\
% %  \cline{1-19}
%  \multicolumn{1}{l}{\ding{183} Mitigation} & & & 0.50 & 0.74 & 0.43 & 0.65 & 0.42 & 0.65 & & & 0.51 & 0.70 & 0.47 & 0.65 & 0.45 & 0.64 & & & 0.51 & 0.69 & 0.47 & 0.62 & 0.49 & 0.64 \\
%  \bottomrule
%  \end{tabular}
% \caption{\footnotesize Reasoning performances on our case study I -- cyber threat intelligence. Query structures are named as {\it path num}--{\it complexity level}, see Figure \mref{fig:query:struc}. \label{tab:case1:benign}}}
% \end{table*}


% \subsection{Attacks}
% To our best knowledge, this work is the first to discuss practical security issues on reasoning systems. We thus compare attacks with different capabilities of attack vectors:
% \begin{mitemize}
% \setlength\itemsep{0.5pt}
% \item $\vect{SA}_{\vect{kgp}}$ -- The \underline{s}tand\underline{a}lone \kgp attack. The attacker is only accessible to \kg as a malicious contributor. A poisoned \kg affects downstream embedding and reasoning without further manipulation of the \kgp attacker.
% \item $\vect{SA}_{\vect{lqe}}$ -- The \underline{s}tand\underline{a}lone \lqe attack. The attacker locates at downstream use cases, thus only affects query contents, including anchor entities and logical structures.
% \item $\vect{CoP}$ -- The \underline{c}o-\underline{o}ptimization attack between \kgp and \lqe, where the downstream \lqe attacker returns specific anchor entities to \kgp attacker for stronger poisoning. Both \kgp and \lqe co-optimize their attacks on a substitute system.
% \end{mitemize}

% We also evaluate on $\ssub{Q}{tar}$ without any attacks as one baseline comparison, to see what are the performance variations with/without attacks.

%\subsection{Evaluation Metrics}

% We use three metrics to evaluate reasoning performances and attacks:
% ({\em i}) \textbf{\textit{MRR}} evaluates the mean reciprocal ranks of all answers among all queries. This metric concerns a global rank quality of reasoning answers. 
% ({\em ii}) \textbf{\textit{HIT@K}} evaluates whether top-$K$ results contain ground-truth answers. For each query, this metric gives a binary indication (0/1). We average those binary results and get a global hits ratio.
% ({\em iii}) \textbf{\textit{NDCG@K}} evaluates the ranking quality of top-$K$ results with the NDCG metric\mcite{}\ting{cite sth}, which is more strict than {\it HIT@K} since positions of ground-truth answers in top-$K$ ranks affects its value.

% The definition is:
% \begin{equation}
% \begin{split}
% \begin{gathered}
%     \text{MRR} = \frac{1}{|Q|} \sum_{q \in Q}^{} \frac{1}{|A|} \sum_{j=1}^{|A|} \frac{1}{rank\left(A\left[j\right]\right)}
% \end{gathered}
% \end{split}
% \label{eq:mrr}
% \end{equation}

% \noindent
% each query $q \in Q$ has an answer set $A$. Thus we first calculate the mean reciprocal rank of each answer for each $q$, then get the query-level mean value.



%\vspace{2pt}
\begin{table}[!ht]
\setlength\extrarowheight{1pt}
\centering
\setlength{\tabcolsep}{2pt}
{\footnotesize
\begin{tabular}{ lclclclclcr}
%  \toprule
% \Xhline{1.5\arrayrulewidth}
 Setting & & Studied cases & & Applications & & Model & & \multicolumn{3}{l}{Results} \\ 
    % \hline
    \cmidrule(){1-11}
    ontological & & I. cyber threat & & \ding{182} Threat Code & & \multirow{2}{*}{Query2Box} & & 0.61 & &  0.76 \\ 
    reasoning & & intelligence & & \ding{183} Mitigation & & &  & 0.47 & &  0.66 \\
    % \hline
    \cmidrule(){1-11}
    relational & & II. drug & & \ding{182} Drug-Disease & & GQE & & \multicolumn{3}{c}{0.73} \\ 
    reasoning & & repurposing & & \ding{183} Drug-Gene & & + R-GCN & & \multicolumn{3}{c}{0.77} \\
    %  \bottomrule
 \end{tabular}
\caption{\footnotesize Two studied reasoning scenarios and their performances. For cyber intelligence, results are MRR (left) and NDCG@5 (right); for drug repurposing, results are HIT@1. \label{tab:benign:all}}}
\end{table}

%\vspace{2pt}


==> todolist.tex <==
(1) ndcg citation 换一下
(2) typo: Beamsearch plot STEP1: "closest"
        STEP3: embeddings are
